HIPPODROME: Data Race Repair using Static Analysis Summaries

Implementing bug-free concurrent programs is a challenging task in modern software development. State-of-the-art static analyses find hundreds of concurrency bugs in production code, scaling to large codebases. Yet, fixing these bugs in constantly changing codebases represents a daunting effort for programmers, particularly because a fix in the concurrent code can introduce other bugs in a subtle way. In this work, we show how to harness compositional static analysis for concurrency bug detection, to enable a new Automated Program Repair (APR) technique for data races in large concurrent Java codebases. The key innovation of our work is an algorithm that translates procedure summaries inferred by the analysis tool for the purpose of bug reporting, into small local patches that fix concurrency bugs (without introducing new ones). This synergy makes it possible to extend the virtues of compositional static concurrency analysis to APR, making our approach effective (it can detect and fix many more bugs than existing tools for data race repair), scalable (it takes seconds to analyse and suggest fixes for sizeable codebases), and usable (generally, it does not require annotations from the users and can perform continuous automated repair). Our study conducted on popular open-source projects has confirmed that our tool automatically produces concurrency fixes similar to those proposed by the developers in the past.

==> FixMapping.tex <==
\section{A Categorization of Infer Warnings} 
\begin{figure*}
	\centering
	\includegraphics[width=\textwidth]{fig/unportectedwrite1.pdf}
	\vspace{-21.9mm}
	\caption{Unprotected Write.\label{fig:war1}}
\end{figure*} 
In this section, we provide the categorization of Infer warnings and link them with a potential fix.
\subsection{Unprotected Write}
One of the frequent warnings generated by Infer is \emph{Unprotected write}. Infer reports this warning whenever a method writes to a field outside of synchronization. This issue originates when multiple threads write to the reported variable simultaneously, and hence a few of them may read an unintended value of this variable. Figure~\ref{fig:war1} shows one of such warnings. The second part of the figure presents the essential information from this warning.

A straight forward (local) fix, considering only this warning, would lock the Line 31. However, there are some facts to consider about this fix:
\begin{itemize}
\item Location of the Lock: A synchronized lock will make the critical field update consistent among other threads. Thus, it should be safe to lock this statement.
\item Selection of the Lock object: Ideally, a lock should not introduce a deadlock. There may be two situations where an incorrect lock could cause a deadlock: 1. We are introducing the lock inside a synchronized method/block. 2. We are introducing the lock in a method invoked from a synchronized method/block. If at least one of these two conditions apply then, we need to care for the lock we introduce. Figure~\ref{fig:deadlock} introduces a context-insensitive solution. The basic idea is to create a map of all lock objects to their inner-most lock object. For example, the initial map contains lock mappings before the new lock (as a part of the fix) is introduced. After the new lock is added, the map is updated to add a new mapping. A deadlock inducing condition can be verified by checking that the new (key-value) pair is not equal to any prior (value-key) pair (in the reverse order). The primary intention is to avoid introducing a new lock that will result in the following order: (lock 1 -> lock 2) and (lock 2 -> lock 1). 

In the scenario where no deadlock condition is present (as in this example), we can safely introduce a lock to statement 31. A potential fix of the above warning could be:\newline \textit{synchronized(new Object()) \{ accounts[accountNumber].setBalance (temp); \}}
%If none of them applies then we can introduce the lock with the field object
\end{itemize}

\begin{figure*}
	\centering
	\includegraphics[width=\textwidth]{fig/deadlock.pdf}
	\vspace{-21.9mm}
	\caption{Context-insensitive Deadlock Check.\label{fig:deadlock}}
\end{figure*}



\begin{figure*}
\centering
\begin{subfigure}{\textwidth}
	\centering
	\includegraphics[width=\textwidth]{fig/ReadWrite.pdf}
	\vspace{-38.9mm}
	\caption{Read/Write Race.\label{fig:ReadWrite}}
\end{subfigure}%
\quad
\begin{subfigure}{\textwidth}
	\centering
	\includegraphics[width=\textwidth]{fig/ReadWrite2.pdf}
	\vspace{-40.9mm}
	\caption{Read/Write Race related Unprotected Write.\label{fig:ReadWrite2}}
\end{subfigure}
\caption{Related Warnings}
\label{fig:test}
\end{figure*}


\subsection{Read/Write Race} Read/Write race is another frequent warning reported by Infer. Figure~\ref{fig:ReadWrite} shows one of such warnings. This issue originates when a method reads a field that may be modified parallelly in another thread. As a result, the warning contains additional information about the method that can write the variable being read. We have denoted this method as \emph{'Conflicting Method`)} in Figure~\ref{fig:ReadWrite}.

A straight forward fix would lock the Line 29. However, in addition to the precautions taken for the \emph{' Unprotected Write`}, we need to consider a few additional points. We have an additional piece of information about the \emph{' Conflicting Method`}. The first task would be to locate the corresponding field update statement in the \emph{' Conflicting Method`}.
If the statement is not synchronized, then we should have another infer warning in the \emph{' Conflicting Method`} about  \emph{' Unprotected Write`} to the same field. This warning will help in locating the field update. Figure~\ref{fig:ReadWrite2} shows the corresponding \emph{' Unprotected Write`} warning for \emph{' Read/Write Race`} in Figure~\ref{fig:ReadWrite}. Please note that we should use the same lock in both methods for the read and write statements.

 If this statement is synchronized, then Infer will not report the \emph{' Unprotected Write`} warning (Figure~\ref{fig:ReadWrite2}). In this case, we need to use program analysis techniques to find the exact location of the update. However, Infer should already have this information. Please note that we need to use the same lock as in the update statement for Line 29 to maintain consistency. 

\subsection{The Overall Picture}
Figure~\ref{fig:cust} presents the CustomerInfo program for which we described the warnings in earlier sections. The blue color arrows mark the related \emph{Read/Write Race} and \emph{Unprotected Write}. For example, \emph{Read/Write Race} in Line 22 is related to \emph{Unprotected Write} in Line 24 (as per Infer warning). Table~\ref{tab:my-table} describes the summary of locks introduced as described in the previous section. A closer look at this table reveals that all of these warnings are related to one field (column 'Field Requiring Lock`), and the locking object should be the same for all lines. In general, the same locks on each line should work; however, in this particular case, locks can also be applied to multiple lines, e.g., from Line 22 to 25. We need to discuss this.

%\begin{figure*}
%	\centering
%	\includegraphics[width=\textwidth]{fig/DataRace.pdf}
%	\vspace{-21.9mm}

%	\caption{CustomerInfo Program\label{fig:cust}}
%\end{figure*}


\begin{table*}[]
\caption{A Summary of the Lock Introduced}
\label{tab:my-table}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\textbf{Id} & \textbf{Warning Type} & \textbf{Modified Method}       & \textbf{Field Requiring Lock}  & \textbf{Location of Lock} & \textbf{Lock Object} \\ \hline
1           & Unprotected Write     & CustomerInfo.deposit(int, int) & this.accounts.{[}\_{]}.balance & Line 31                   & accounts or new lock \\ \hline
2           & Read/Write Race       & CustomerInfo.deposit(int, int) & this.accounts.{[}\_{]}.balance & Line 29                   & accounts or new lock \\ \hline
3           & Unprotected Write     & CustomerInfo.withdraw(int,int) & this.accounts.{[}\_{]}.balance & Line 24                   & Same as Id 2         \\ \hline
4           & Read/Write Race       & CustomerInfo.withdraw(int,int) & this.accounts.{[}\_{]}.balance & Line 22                   & Same as Id 3         \\ \hline
\end{tabular}
\end{table*}

\subsection{Comparison to PFix's Fix} PFix requires multiple execution traces, including the buggy execution, to detect this problem. However, in this particular example, the threads do not execute \emph{withdraw} method, and hence PFix does not consider any races in the \emph{withdraw} method. However, this is a more significant problem as execution traces are often incomplete, and PFix will miss many of such problems. However, Infer proactively detects these cases, and thus we cover many unintended and hidden cases. Figure~\ref{fig:fixvsus} shows a comparison of PFix's fix vs ours. 


%\begin{figure*}
%	\centering
%	\includegraphics[width=\textwidth]{fig/pfixvsus.pdf}
%	\vspace{-21.9mm}
%	\caption{CustomerInfo Program\label{fig:fixvsus}}
%\end{figure*}

\begin{figure*}
\centering
\begin{subfigure}{\textwidth}
	\centering
\includegraphics[width=\textwidth]{fig/DataRace.pdf}
\vspace{-35.9mm}
	\caption{CustomerInfo Program\label{fig:cust}}
\end{subfigure}%
\quad
\begin{subfigure}{\textwidth}
	\centering
\includegraphics[width=\textwidth]{fig/pfixvsus.pdf}
	\vspace{-38.9mm}
	\caption{Fix Comparision\label{fig:fixvsus}}
\end{subfigure}
\caption{Fix Example}
\end{figure*}

==> FixStrategy.tex <==
\section{Summaries to Fixes}
Summaries contain multiple \emph{access snapshots} for a method. For a given statement in a method, a snapshot includes the nature of the data access, lock patterns, and whether multiple threads can access this statement. Comparing various access patterns give insights on concurrent data modifications across the same or different methods. In Section, we determined the race inducing conditions over two access snapshots.  In the following, we split the race condition into different categories. These categories help in localizing the fix patterns.
\subsection{Read/Write Race}
 Read/Write race is a frequent cause of data race in a concurrent program. This issue originates when a thread reads a shared field that may be modified parallelly by another thread. Given two access snapshots, we  formally define the read/write race as:
\begin{definition}
Let A1 = $\{\csummary{\spath_1}{k_1}{L_{a1}}{L_s1}{t_1}{o_1}{n_1}{\trace_1} \mid k_1 \in \{ \rrd,\rwr \}\}$ and A2 = $\{\csummary{\spath_2}{k_2}{L_{a2}}{L_s2}{t_2}{o_2}{n_2}{\trace_2} \mid k_2 \in \{ \rrd,\rwr \}\}$ be two race inducing accesses. These accesses can be further classified into read/write race if:
\begin{itemize}
\item $({k_1} == rd \; \&\& \; {k_2} == wr) \; \| \; ({k_1} == wr \;\&\&\; {k_2} == rd\})$, and
\item $(L_{a1} \neq L_{a2}) \; \| \; (L_{a1} == \phi ==  L_{a2})$
\end{itemize}
\end{definition} 
Intuitively, if a shared variable is being read and modified concurrently without a lock or with disjoint locks, then a read/write race transpires. The corresponding read and write operations can be either in the same method or even in different methods. Depending on the location of these operations, one or multiple locks may be required to fix these races. In the following, we discuss the fix scope and strategies:
\subsubsection{Fix Scope and Strategies}
\begin{figure}
\setlength{\belowcaptionskip}{-10pt}
$\pi_1 = \pi_2$ $\bigtimes$\\
$\land$ $(k_1 = rd \land k_2 =wr) \| (k_1 = wr \land k_2 = rd) $ $\bigtimes$\\
$\land$ $(L_{a1} \neq L_{a2}) \; \| \; (L_{a1} = \phi =  L_{a2})$ \Large{$\checkmark$}\normalsize{}\\
$\land$ $t_1 \sqcup t_2 = AnyThread$ $\bigtimes$\\
$\land$ $o_1 \neq Owned \land o_2 \neq Owned$ $\bigtimes$
\caption{Read/Write Race Inducing Conditions. \label{fig:fixscope}}
\end{figure}

Fix scope signifies the type of changes to eliminate the race condition. As is, multiple states need to match for a race; consequently, it would suffice to remove one or more race inducing conditions. Figure~\ref{fig:fixscope} describes the possibilities of offsetting various conditions required for a read/write race. It is clear that changing the reads and writes of a field (k), and its path ($\spath$) is not viable, as it could change the program behavior altogether. Restricting the thread access  ($\mathit{t_1 \sqcup t_2 \neq AnyThread}$) would sacrifice the concurrency, and thus it is not a valid solution. Similarly, changing the ownership of the shared field may change the intended behavior of the program. Finally, changing the lock patterns seems to be the most practical fix in this case. 

\textit{Lock Patterns} There can be multiple scenarios of how two access snapshots lock the shared field:
\begin{enumerate}[label=(\Alph*)]
\item Different lock objects are guarding the read and write access to the shared field.
\item There is a lock for reading a field, but no lock for writing.
\item There is a lock for writing a field, but no lock for reading. 
\item There are no locks, i.e., $L_{a1} == \phi ==  L_{a2}$
\end{enumerate}

\begin{figure*}
\begin{subfigure}[t]{0.5\textwidth}
if $(L_{a1} = l1) \land L_{a2} = l2)$ then \\
$PC_1$: $L_{a1} = l1 = L_{a2}$ \\
$PC_2$: $L_{a1} = l2 = L_{a2}$ \\
$PC_3$: $L_{a1} = l1 \land L_{a2} = l2 + l1$ \\
$PC_4$: $L_{a1} = l1 + l2 \land L_{a2} = l2$ \\
\caption{Case A.}
\end{subfigure}
\begin{subfigure}[t]{0.5\textwidth}
if $(L_{a1} = l1) \land L_{a2} = null)$ then \\
$PC_1$: $L_{a1} = l1 = L_{a2}$
\caption{Case B}
\end{subfigure}
\vspace{-12mm}
\flushright
\begin{subfigure}[t]{0.5\textwidth}
if $(L_{a1} = null) \land L_{a2} = null)$ then \\
$PC_1$: $L_{a1} = l_* = L_{a2}$
\caption{Case C}
\end{subfigure}
\caption{Potential Fix Candidates. $PC$ denotes Patch Candidates\label{fig:fixpat}}
\end{figure*}
Figure~\ref{fig:fixpat}  shows potential fix candidates corresponding to each lock pattern. Case A has four potential fix candidates, while case B, C, and D have one fix candidate. However, selecting a fix candidate requires answering following questions.
\begin{itemize}
\item Which lock object to use? For example, in Case A, whether to use fix 1 (lock $l1$) or 2 (loc $l2$).
\item How to avoid deadlocks when adding additional locks? For example, while introducing fix candidates 3, 4 for Case A, how to avoid deadlock?
\end{itemize}

\textit{Which Lock Object?} There is no best solution for selecting a lock object, except it should prevent deadlocks. However, we define Function~\ref{eq:1} to choose a lock object based on its distance from the path($\spath$). The distance signifies the object equivalence of lock object to the $\spath$. For example, for a given path $this.A.b$, the first preferred lock object is $this.A.b$, the second preferred lock object is $this.A$, and finally the third preferred lock object is $this$. 

\begin{equation} \label{eq:1}
 \mathcal{H} (l) = \left.
	\begin{cases}
		l1, & \text{if $l1$ is closer to $\spath$ than $l2$} \\
		l2, & \text{if $l2$ is closer to $\spath$ than $l1$} \\
	    l1+l2, & \text{otherwise } 
	\end{cases}
	\right\} 
 \end{equation}

\textit{Avoiding Deadlocks:}
Ideally, adding a new lock should not introduce a deadlock. However, the addition of a new lock is prone to deadlocks. For example, consider a method with a synchronized block with a lock object $l1$, and this block has an internal synchronized block with a lock object $l2$. Similarly, a different method has a synchronized block with a lock object $l2$, and our fix adds a new synchronized lock $l1$ inside this synchronized block. Consequently, the repair may introduce a deadlock as now the locks are in the following order: $(l1 \rightarrow l2)$ and $(l2 \rightarrow l1)$. Hence, it becomes crucial to take precautions to avoid deadlocks while adding a new lock. 

To avoid deadlocks, we propose a context-insensitive solution.  

==> PFixBenchmark.tex <==
The aim of this study is to provide more insights into the cases where Infer fails to report a warning. We have created this report on \pfix's dataset, which also includes cases from several other benchmarks such as calFuzzer. In the following, we describe a few cases and provide an initial understanding of why Infer failed.

\begin{table}[]
\caption{Results of Infer on \pfix Benchmark. AV -- Atomicity Violation, CB -- Consistency bug, DR -- Data Race} 
\label{tab:rq1}
%\vspace{2mm}
\begin{adjustbox}{width=\width}
\centering
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
{\color[HTML]{000000} \textbf{Id}} & {\color[HTML]{000000} \textbf{Program Name}} & {\color[HTML]{000000} \textbf{\#line}} & {\color[HTML]{000000} \textbf{type}} & {\color[HTML]{000000} \textbf{Infer Detection}}  \\ \hline
1                                  & account                                      & 102                                    & AV                  & Fail                                                                                                                           \\ \hline
2                                  & accountsubtype                               & 138                                    & AV                  & Fail                                                                                                                           \\ \hline
3                                  & airline                                      & 51                                     & AV                  & Success                                                                                                                           \\ \hline
4                                  & alarmclock                                   & 206                                    &                     & Success                                                                                                                                  \\ \hline
5                                  & atmoerror                                    & 48                                     & DR                  & Success                                                                                                                          \\ \hline
6                                  & buggyprogram                                 & 258                                    & AV                  & Success                                                                                                                            \\ \hline
7                                  & checkfield                                   & 41                                     & AV                  & Fail                                                                                                                           \\ \hline
8                                  & consisitency                                 & 28                                     & CB                  & Success                                                                                                                           \\ \hline
9                                  & critical                                     & 56                                     & AV                  & Fail                                                                                                                          \\ \hline
10                                 & datarace                                     & 90                                     & DR                  & Success                                                                                                                          \\ \hline
11                                 & even                                         & 49                                     & AV                  & Success                                                                                                                           \\ \hline
12                                 & hashcodetest                                 & 1258                                   & AV                  & Success                                                                                                                           \\ \hline
13                                 & linkedlist                                   & 204                                    & AV                  & Success                                                                                                                            \\ \hline
14                                 & mergesort                                    & 270                                    & AV                  & Success                                                                                                                               \\ \hline
15                                 & pingpong                                     & 130                                    & DR                  & Fail                                                                                                                          \\ \hline
16                                 & ProducerComsumer                             & 144                                    &                     & Fail                                                                                                                              \\ \hline
17                                 & reorder2                                     & 135                                    & CB                  & Success                                                                                                                            \\ \hline
18                                 & store                                        & 44                                     & AV                  & Success                                                                                                                           \\ \hline
19                                 & stringbuffer                                 & 416                                    & AV                  & Fail                                                                                                                            \\ \hline
20                                 & wrongLock                                    & 73                                     & AV                  & Fail                                                                                                                         \\ \hline
21                                 & wrongLock2                                   & 36                                     & DR                  & Success                                                                                                                           \\ \hline
\end{tabular}
\end{adjustbox}
\end{table}

\subsubsection{Account}
\begin{figure*}
	\centering
	\includegraphics[width=\textwidth]{fig/ConcurrencyExamples.pdf}
	\caption{Test Id 1, account. Atomic violation.\label{fig:arc}}
\end{figure*} 
Figure~\ref{fig:arc} shows relevant parts of a very basic bank account program. The program provides basic accounting functionalities such as deposit money into an account (Line 3-5). However, this program experiences an atomicity violation while transferring money from one account to the other. The bug manifestation is demonstrated by creating ten accounts threads (``A" to ``J") with an initial amount of 100 dollars (Line 36-38). These account threads are run (Line 25-33) to perform accounting functions such as transfer money from one account to another. A correct execution should leave each account with 300 dollars at the end. However, running this program multiple times reveals that in some executions few accounts do not have 300 dollars. While all the functions \emph{(deposit, withdraw, and transfer)} in the Account class are \emph{synchronized}, they all modify related variables (amount) without \emph{synchroniztion}. In the \emph{run} method of each thread (Line 25), each thread accesses the critical section of other threads. For example, the scenario where the thread C is transferring amount to the account D (Line 27) and at the same time D is withdrawing (Line 30) results in a data race for the amount in D. In particular, the scenario where one thread is either depositing or withdrawing and the other thread transfer money to it causes an atomic violation. A potential fix puts a lock at Line 13 to make the account modification atomic (\textit{+=} is not an atomic operation).

\paragraph*{Infer's Warning} We ran Infer on this program under two configurations: 1. Without \emph{@ThreadSafe} annotation, and 2. With \emph{@ThreadSafe} annotation in \emph{Account} and \emph{ManageAccount} class. In the first case, Infer reported no warnings. This may be due to the reason that Infer doesn't detect bugs involving dual-lock configuration. In the second case (With \emph{@ThreadSafe}), Infer reported five warnings in \emph{ManageAccount}, however, these warnings were mainly because the constructor (Line 20) and the \emph{run} method (Line 25) are not \emph{synchronized}. The most relevant warning states \emph{ Read/Write race. Non-private method `void ManageAccount.run()` reads without synchronization from `account.ManageAccount.accounts.[\_]`. Potentially races with write in method `ManageAccount(...)`.}. This warning reports that a read/write violation of the \emph{accounts} variable in the \emph{run} method and the constructor. A thorough analysis of these bugs did not lead to the reported bug.
\paragraph*{Post mortem analysis} This is a tricky case. Analysis should detect that each bank account thread could concurrently access the critical data (via \emph{accounts} variable) of different threads via the \emph{transfer} function (Line 27, 29, 32). In addition, analysis should be able to connect that the \emph{transfer} method can run in parallel to \emph{withdraw} and \emph{deposit}.  

\subsubsection{Checkfield}
Figure~\ref{fig:checkfield} shows parts of the checkfield program. This is a fairly simple program with two threads t1 and t2. Both threads try to modify the shared variables number and num2 (of class InstanceExample). As there is no synchronization among these threads, there is an atomic violation among the statements marked red. A potential fix is to lock the modification of shared variables on both the threads (marked green).
\paragraph*{Infer's Warning} We ran Infer on this program under two configurations: 1. Without \emph{@ThreadSafe} annotation, and 2. With \emph{@ThreadSafe} annotation. In the first case, Infer reported no warnings, this is because there are no synchronization statements present. In the second case, Infer reported three warnings. However, none of these warnings were pointing towards the actual problem. The most relevant warning is shown in Figure~\ref{fig:checkfield}.
\paragraph*{Post mortem analysis} This is a straight forward case. Infer should have detected this case. My initial thoughts were that this might be because we are putting @ThreadSafe in the main class. To avoid this, I separated the creation of threads to another class. However, then infer reported no warnings at all, even with @ThreadSafe annotation. This leaves us with a possibility that Infer does not understand the way threads are created in this example, i.e., using new Thread().   
%\begin{figure*}
%	\centering
%	\includegraphics[width=\textwidth]{images/checkfield.pdf}
%	\caption{Test Id 7, checkfield. Atomic violation.\label{fig:checkfield}}
%\end{figure*} 

\subsubsection{WrongLock}
Figure~\ref{fig:wronglock} shows parts of the wrongLock program. This program demonstrates the ineffectiveness of using different locks to the same variable. The \emph{WrongLock} class creates two methods \emph{A} and \emph{B}. Method \emph{A} increments the value of instance variable \emph{data} under the \emph{data} lock, while the method \emph{B} applies same operation under lock \emph{this}. As is, these locks are different, and hence different threads can increment the value of \emph{data} simultaneously. This may result in an unexpected value of \emph{data}. A potential fix is to use the same lock (marked with green).
\paragraph*{Infer's Warning} We ran Infer on this program under two configurations: 1. Without \emph{@ThreadSafe} annotation, and 2. With \emph{@ThreadSafe} annotation. In both cases, Infer reported no warnings.  
\paragraph*{Post mortem analysis} There may a possibility that Infer does not detect cases where different locks are used. This issue needs to be looked carefully because wrong locks can produce deadlocks. Moreover, this could also be a frequent issue in real-world projects.
% \begin{figure*}[hbt!]
	%\centering
%	\includegraphics[width=\textwidth]{images/WrongLock.pdf}
%	\caption{Test Id 20, wrongLock. Atomic violation.\label{fig:wronglock}}
%\end{figure*} 


\begin{figure*}
\centering
\begin{subfigure}{\textwidth}
	\centering
	\includegraphics[width=\linewidth]{fig/checkfield.pdf}
	\caption{Test Id 7, checkfield. Atomic violation.\label{fig:checkfield}}
	\label{fig:sub1}
\end{subfigure}%
\quad
\begin{subfigure}{\textwidth}
	\centering
	\includegraphics[width=\linewidth]{fig/WrongLock.pdf}
	\caption{Test Id 20, wrongLock. Atomic violation.\label{fig:wronglock}}
	\label{fig:sub2}
\end{subfigure}
\\
\todo{This is ginormous! Please, reduce to a minimal example and outline the important parts.}
\caption{Special Cases where Infer Fails}
\label{fig:test}
\end{figure*}


==> fig/abstractdomain-bugs.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% ABSTRACT DOMAIN BUGS %%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\setlength{\belowcaptionskip}{-10pt}
%\setlength{\abovecaptionskip}{-10pt}
\centering
\[
\!\!\!\!
{\small
\begin{array}{l@{\ \ }l@{\ \ }c@{\ \ }l}
  \text{bug} & \bug \in \bugsad & = & 
  \{ \snapshot \mid write\_race (\snapshot)  = \True  \} ~\cup
  \\
  &&&
   \{ (\snapshot_1, \snapshot_2) \mid race (\snapshot_1, \snapshot_2)  = \True  \}
  \\[2pt]
  \text{patch} & \patch & = & \{(\trace,\stmt_f,\stmt_t)\}
  % \\[2pt]
  % \text{domain} & d \subseteq \mathcal{D} & = & \mathcal{L} \times \mathcal{T}
  %                                               \times \mathcal{E} \times \mathcal{A}
\end{array}
}
\]
\caption{Abstract Domain for Patch Generation.}
\label{fig:abstract-domain-bugs}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper"
%%% End:


==> fig/hello-world.tex <==

\begin{figure}[t]
\setlength{\belowcaptionskip}{-10pt}
%\setlength{\abovecaptionskip}{-10pt}
\centering
\begin{lstlisting}[style=numbering]
public class WrongLock {
  Data data;
  public void A() {
    synchronized (data) {
      int x = data.value;
      data.value++;
      if (data.value != (x + 1))
        throw new RuntimeException("bug found");
     }
  }
  public void B() {
    synchronized (this) { data.value++; }
  }
}
\end{lstlisting}
\caption{Race example which highlights: race, variable scope, differnt locks
  (see PFix's benchmark - wronglock)}
\label{fig:wronglock}
\end{figure}


==> fig/lang.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% SIL PROGRAMMING LANGUAGE %%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{figure}[t]
% \setlength{\belowcaptionskip}{-10pt}
% %\setlength{\abovecaptionskip}{-10pt}
% \centering
% \[
% \!\!\!\!
% {\small
% \begin{array}{r@{\ \ }c@{\ \ }l}

%   E & ::= & x \mid nil \mid c \\[2pt]
%   B & ::= & E=E \mid E\neq E  \\[2pt]
%   S & ::= & x:=E
%             \mid X:=E \leftarrow t
%             \mid E \leftarrow t :=E
%             \mid x= new()
%             \mid dispose(E)
%   \\[2pt]
%   C & ::= & S
%             \mid C;C
%             \mid \ifz(B) \{C\} \elsez \{C\}
%             \mid \whilez(B)[I]\{C\}
%   \\[2pt]
%   &&
%             \mid f(\overrightarrow{x},\overrightarrow{E})
%             \mid f(\overrightarrow{x},\overrightarrow{E}) || f(\overrightarrow{x},\overrightarrow{E})
%             \mid \withz~ r ~\whenz(B){C}
% \end{array}
% }
% \]
% \caption{The Grammer of Smallfoot Intermediate Language. \ac{SIL or Java?}}
% \label{fig:lang}
% \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% CORE PROGRAMMING LANGUAGE %%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[t]
\setlength{\belowcaptionskip}{-10pt}
%\setlength{\abovecaptionskip}{-10pt}
%\centering
\[
\!\!\!\!
{\small
\begin{array}{l@{\!\!}r@{\ }c@{\ }l@{\ }c@{\ \ }l}
  \text{variables} & x & \in & \multicolumn{2}{@{}l@{\!\!}}{\mathrm{Var} \cup \{ \mcode{this} \}}  \\
  \text{field names} & f & \in & \mathrm{Field} && \\
  \text{modifiers} & \modif & \in & \multicolumn{3}{@{}l@{\!\!}}{\{
                                   \text{\code{static},
                                   \code{volatile}, \code{private}, \ldots }\} }\\
 \text{types} & t & \in & \mathrm{Type} && \\
  \text{method names~~~} & m & \in & \mathrm{Meth} && \\
  \text{access paths} & \spath & \in & \mathrm{Path} & ::= & \mathrm{Var} \times
                                                        \mathrm{Field^*} \\
  \text{expressions} & e & \in & \mathrm{Exp} & ::= & \spath \mid \spath.f \\
  \text{commands} & c & \in & \mathrm{Cmd} & ::= & \spath_1 = \spath_2
                                            \mid \spath = \callz\,
                                               m(\overrightarrow{e}) \mid \\
  &&&&&                                              \modif~t~ x \mid \modif~t~ x  = e \mid \\                                                                                
  &&&&&                                              \text{\sync{x}}\{\  \stmt  \ \} \\
  \text{statements} & \stmt & \in & \mathrm{Stmt} & ::= & c_1 ;  c_2 \mid \ldots 
\end{array}
}
\]
\caption{The core language.}
\label{fig:lang}
\end{figure}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper"
%%% End:


==> macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Packages
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\usepackage{amsmath,amssymb,amsfonts}
\usepackage{amsmath,amsfonts}
\usepackage{booktabs} % For formal tables
%\usepackage[colorlinks=true]{hyperref}
%\usepackage{cite}
\usepackage[10pt]{moresize}
\usepackage{graphicx}
\usepackage[english]{babel}
\usepackage{dsfont}
\usepackage{latexsym}
\usepackage{tcolorbox}
\usepackage{listings}
\usepackage{float}
\usepackage{multirow}
\usepackage[scaled]{helvet}
%\usepackage[noend]{algorithmic}
\usepackage[noend]{algpseudocode}
\usepackage{mathrsfs}
\usepackage[linesnumbered, ruled, lined]{algorithm2e}  %block lines looks annoying
\usepackage{mathpartir}
\usepackage{mathtools}
\usepackage{dsfont} 
\usepackage{stmaryrd}
\usepackage{url}
\usepackage{textcomp} 
%\usepackage{titlesec}
\usepackage{bbm}
\usepackage{verbdef}
\usepackage{xspace}
\usepackage{verbatim}
\usepackage{lipsum}
\usepackage{wrapfig}
\newcounter{tags}
\usepackage{enumitem}
\usepackage{pifont}
\usepackage{varwidth}
\usepackage{xpatch}
\usepackage{multirow}
\usepackage{xcolor}
\usepackage[export]{adjustbox}
\usepackage{caption}
\usepackage{subcaption}
%\usepackage{lineno}

%%% Yes! Pretty monospace fonts, finally! Hell yeah!
\usepackage[varqu]{zi4}

\usepackage{flushend}

\usepackage{tikz}
\usetikzlibrary{calc,positioning,math, arrows, shapes}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}

\def\sectionautorefname{Sec.}
\def\subsectionautorefname{Sec.}
\def\subsectionautorefname{Sec.}
\def\subsubsectionautorefname{Sec.}
\def\figureautorefname{Fig.}
\def\tableautorefname{Tab.}
\def\equationautorefname{Eq.}

\AtBeginDocument{%
  \providecommand\BibTeX{{%
    \normalfont B\kern-0.5em{\scshape i\kern-0.25em b}\kern-0.8em\TeX}}}

\setlist[itemize]{topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex,itemindent=0pt,leftmargin=8pt}
\lstset{language=C,keywordstyle={\bfseries \color{blue}}}
%\linenumbers
%\renewcommand\linenumberfont{\normalfont\tiny\sffamily\color{red}}



\definecolor[named]{ACMBlue}{cmyk}{1,0.1,0,0.1}
\definecolor[named]{ACMYellow}{cmyk}{0,0.16,1,0}
\definecolor[named]{ACMOrange}{cmyk}{0,0.42,1,0.01}
\definecolor[named]{ACMRed}{cmyk}{0,0.90,0.86,0}
\definecolor[named]{ACMLightBlue}{cmyk}{0.49,0.01,0,0}
\definecolor[named]{ACMGreen}{cmyk}{0.20,0,1,0.19}
\definecolor[named]{ACMPurple}{cmyk}{0.55,1,0,0.15}
\definecolor[named]{ACMDarkBlue}{cmyk}{1,0.58,0,0.21}

\makeatletter
\def\arcr{\@arraycr}
\makeatother

%% Math enumerations

\makeatletter
\newcommand{\mtmathitem}{%
\xpatchcmd{\item}{\@inmatherr\item}{\relax\ifmmode$\fi}{}{\errmessage{Patching of \noexpand\item failed}}
\xapptocmd{\@item}{$}{}{\errmessage{appending to \noexpand\@item failed}}}
\makeatother
\newenvironment{mathitem}[1][]{%
\itemize[#1]\mtmathitem}{$\endlist}                    %$
\newenvironment{mathenum}[1][]{%
\enumerate[#1]\mtmathitem}{$\endlist}                  %$
\newenvironment{mathdesc}[1][]{%
\description[#1]\mtmathitem}{$\endlist}                %$

%%%%%%%%%%%%

% Colors

\definecolor{shadecolor}{gray}{1.00}
\definecolor{ddarkgray}{gray}{0.75}
\definecolor{darkgray}{gray}{0.30}
\definecolor{light-gray}{gray}{0.87}
\newcommand{\whitebox}[1]{\colorbox{white}{#1}}
\newcommand{\graybox}[1]{\colorbox{light-gray}{#1}}
\newcommand{\darkgraybox}[1]{\colorbox{ddarkgray}{#1}}
\newcommand{\gbm}[1]{\graybox{${#1}$}}
\newcommand{\Inv}{\text{\textsc{Inv}}}
\newcommand{\TPCInv}{\text{\textsc{TPCInv}}}
\newcommand{\litho}{\textsf{Litho}\xspace}

\newcommand{\hsh}{\mathit{h}}
\newcommand{\hshs}{\mathit{hs}}

% \newcommand{\ind}{\mathit{\iota}}
% \newcommand{\inds}{\mathit{\overline{\iota}}}
\newcommand{\ind}{\mathit{\iota}}
\newcommand{\inds}{\mathit{{\iota}{s}}}

\newcommand{\fstar}{\text{F}^{\star}}
\newcommand{\etc}{\emph{etc}}
\newcommand{\ie}{\emph{i.e.}\xspace}
\newcommand{\Ie}{\emph{I.e.}\xspace}
\newcommand{\eg}{\emph{e.g.}\xspace}
\newcommand{\Eg}{\emph{E.g.}\xspace}
\newcommand{\vs}{\emph{vs.}\xspace}
\newcommand{\etal}{\emph{et~al.}\xspace}
\newcommand{\adhoc}{\emph{ad hoc}\xspace}
\newcommand{\viz}{\emph{viz.}\xspace}
\newcommand{\dom}[1]{\mathsf{dom}(#1)}
%\newcommand{\im}[1]{\mathsf{im}(#1)}
\newcommand{\im}[1]{{#1}}
\newcommand{\aka}{\textit{a.k.a.}\xspace}
\newcommand{\cf}{\textit{cf.}\xspace}
\newcommand{\wrt}{\emph{wrt.}\xspace}
\newcommand{\Iff}{\emph{iff}\xspace}
\newcommand{\loef}{L\"{o}f}

\newcommand{\denot}[1]{\llbracket{#1}\rrbracket}


\newcommand{\ifext}[2]{\ifdefined\extflag{#1}\else{#2}\fi}
\newcommand{\ifcomm}[1]{\ifdefined\extcomm{#1}\else{}\fi}

% \theoremstyle{remark}
% \newtheorem{example}{Example}[section]

% \theoremstyle{definition}
% \newtheorem{definition}{Definition}[section]

% \theoremstyle{plain}
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{corollary}[theorem]{Corollary}
% \newtheorem{pattern}[theorem]{Pattern}
% \newenvironment{proofsketch}{\trivlist\item[]\emph{Proof sketch}:}%
% {\unskip\nobreak\hskip 1em plus 1fil\nobreak$\square$
% \parfillskip=0pt%
% \endtrivlist}


%\newcommand{\mute}[1]{\ifcomm{#1}}
\newcommand{\mute}[1]{{#1}}
\newcommand{\ccode}[1]{\text{\lstinline[basicstyle=\small\ttfamily]{#1}}}

\newcommand{\tsend}{\mathsf{send}}
\newcommand{\treceive}{\mathsf{receive}}
\newcommand{\tskip}{\mathsf{skip}}

\newcommand{\disel}{{\sc Disel}\xspace}
\newcommand{\withinvr}{{\sc WithInv}\xspace}
\newcommand{\True}{\mathsf{True}}
\newcommand{\id}{\mathsf{id}}
\newcommand{\False}{\mathsf{False}}
\newcommand{\set}[1]{\left\{{#1}\right\}}
\newcommand{\angled}[1]{\langle{#1}\rangle}


%% Specs
\newcommand{\specK}[1]{\ensuremath{\textcolor{blue}{\set{#1}}}}
\newcommand{\pre}[2]{\specK{\lambda {#1}.~{#2}}}
\newcommand{\post}[3]{\specK{\lambda {#1}~{#2}.~{#3}}}
\newcommand{\psep}{\ast}

%% Protocols
\newcommand{\ppr}{\mathcal{P}}
\newcommand{\cpr}{\mathcal{C}}

%% State-space and Transitions
\newcommand{\treq}{\mathsf{Req}}
\newcommand{\tresp}{\mathsf{Resp}}
\newcommand{\acts}{\Send}
\newcommand{\actr}{\Recv}
\newcommand{\trans}[1]{\mathit{#1}}
\newcommand{\To}{\mathit{to}}
\newcommand{\Rs}{\mathit{rs}}
\newcommand{\From}{\mathit{from}}
\newcommand{\args}{\mathit{args}}
\newcommand{\ans}{\mathit{ans}}
\newcommand{\aand}{~\dot{\wedge}~}
\newcommand{\iimp}{~\dot{\Rightarrow}~}
\newcommand{\nneg}{\dot{\neg}}
\newcommand{\aandb}{\&\!\!\!\&}
\newcommand{\oor}{\vee}
\newcommand{\body}{\mathit{body}}
\newcommand{\clients}{\overline{C}}
\newcommand{\servers}{\overline{S}}
\newcommand{\Send}{\mathsf{send}}
\newcommand{\Recv}{\mathsf{recv}}
\newcommand{\csend}[1]{\Send[#1]}
\newcommand{\creceive}[1]{\Recn[#1]}
\newcommand{\lab}{\ell}
\newcommand{\Some}{\mathsf{Some}}
\newcommand{\None}{\mathsf{None}}
\newcommand{\truez}{\mathsf{true}}
\newcommand{\falsez}{\mathsf{false}}

\newcommand{\inject}{\ensuremath{\mathsf{inject}}\xspace{}}
\newcommand{\unitz}{\mathsf{unit}\xspace{}}
\newcommand{\letz}{\mathsf{{\bf let}}\xspace{}}
\newcommand{\inz}{\mathsf{{\bf in}}\xspace{}}
\newcommand{\retz}{\mathsf{{\bf return}}\xspace{}}
\newcommand{\letrecz}{\mathsf{{\bf letrec}}\xspace{}}
\newcommand{\ifz}{\mathsf{{\bf if}}\xspace{}}
\newcommand{\thenz}{\mathsf{{\bf then}}\xspace{}}
\newcommand{\elsez}{\mathsf{{\bf else}}\xspace{}}
\newcommand{\whilez}{\mathsf{{\bf while}}\xspace{}}
\newcommand{\withz}{\mathsf{{\bf with}}\xspace{}}
\newcommand{\whenz}{\mathsf{{\bf when}}\xspace{}}
\newcommand{\newz}{\mathsf{{\bf new}}\xspace{}}
\newcommand{\callz}{\mathsf{{\bf call}}\xspace{}}
\newcommand{\lockz}{\mathsf{{\bf lock}}\xspace{}}
\newcommand{\unlockz}{\mathsf{{\bf unlock}}\xspace{}}
\newcommand{\Active}{\circ}
\newcommand{\Consumed}{\bullet}
\newcommand{\asgn}{\leftarrow}
\newcommand{\vd}[1] {\mathrel{\overset{#1}{\vdash}}}
\newcommand{\blockr}{\mathsf{receive\_req}}
\newcommand{\blockresp}{\mathsf{receive\_resp}}
\newcommand{\osserver}{\mathsf{simple\_server}}
\newcommand{\dserver}{\mathsf{deleg\_server}}
\newcommand{\cclient}{\mathsf{compute}}
\newcommand{\bserver}{\mathsf{batch\_server}}
\newcommand{\mserver}{\mathsf{memo\_server}}
\newcommand{\num}[1]{{\text{{\scriptsize{#1}}}}}
\newcommand{\eqdef}{\triangleq}
\newcommand{\withinv}{\mathsf{WithInv}}
\newcommand{\serv}{\mathit{serv}}
\newcommand{\figsize}{\footnotesize}


% bloomfilter specific
\newcommand{\ncr}[2]{\left(\begin{matrix} #1 \\ #2 \end{matrix} \right)}
\newcommand{\stirlingsnd}[2]{\left\{\begin{matrix} #1 \\ #2 \end{matrix} \right\}}
\newcommand{\ordnat}[1]{\nat_{[0,\ldots,#1-1]}}
\newcommand{\bloomfilter}{\mathit{bf}}
\newcommand{\bff}{\bloomfilter}
\newcommand{\vseq}{\mathit{vs}}
\newcommand{\yseq}{\mathit{ys}}
\newcommand{\xseq}{\mathit{xs}}
\newcommand{\countingbloomfilter}{c\!f}
\newcommand{\bfquery}[2]{#1 \in_? #2}
\newcommand{\bfseen}[1]{I_{#1}}
\newcommand{\fintuple}[2]{{#1}\!-\!\text{tuple} ~ #2}

\newcommand{\nrounds}{\mathit{N_{\text{rounds}}}}
\newcommand{\cgp}{\mathsf{CGP}\xspace}
\newcommand{\cpp}{\mathsf{CPP}\xspace}
\newcommand{\tep}{\mathsf{TEP}_{\!\varepsilon}\xspace}


% Fancy pointers
\newcommand{\ppts}[1]{\mathrel{\overset{#1}{\mapsto}}}
\newcommand{\pmap}{\mathrel{\overset{\text{\!\!\!\tiny{fin}}}{\rightharpoonup}}}
\newcommand{\pfun}{\rightharpoonup}

\newcommand{\world} {\ccode{World}}
\newcommand{\bool} {\ccode{bool}}
\newcommand{\dist}[1] {\ccode{dist} ~ #1}
\newcommand{\bind }{\vartriangleright  }
\newcommand{\sch}{\ccode{seq}~\ccode{RndGen}}
\newcommand{\sched}{\mathit{sc}}
\newcommand{\comp}[1] { \ccode{Comp} ~ #1 }
\newcommand{\prob}[1] { \Pr\left[#1\right]}
\newcommand{\expt}[1] { \text{E}\!\!~\left[#1\right]}
\newcommand{\support}[1] { \Omega ( #1 ) }
\newcommand{\chain}{\mathit{BlockChain}}
\newcommand{\reals} { \mathds{R} }
\newcommand{\nat}{ \mathds{N} }
\newcommand{\bools}{ \mathds{B} }
\newcommand{\addr} {\mathit{addr}}
\newcommand{\worldstep}{\ccode{world_step}}
\newcommand{\nactors}{\mathit{max_{\text{actors}}}}
\newcommand{\tname}[1]{\textsc{#1}\xspace}
\newcommand{\pfix}{\tname{PFix}}
\newcommand{\afix}{\tname{AFix}}
\newcommand{\hfix}{\tname{HFix}}
\newcommand{\grail}{\tname{Grail}}
\newcommand{\footpatch}{\tname{FootPatch}}
\newcommand{\lname}[1]{{\small{\textsf{#1}}}\xspace}
%\newcommand{\lname}[1]{\tname{#1}}
\newcommand{\progname}[1]{{#1}\xspace}
\newcommand{\genprog}{\tname{GenProg}}

% Tools
\newcommand{\inferr}{\tname{Infer}}
\newcommand{\racerd}{\tname{RacerD}}
\newcommand{\tool}{\tname{RacerDFix}}
\newcommand{\logic}{CSL$_{\text{fix}}$\xspace{}}


% Race specific notations
\newcommand{\spath}{\pi}
\newcommand{\trace}{\tau}
\newcommand{\rrd}{\mathbf{rd}}
\newcommand{\rwr}{\mathbf{wr}}
\newcommand{\summary}[7]{\langle #1,#2,#3,#4,#5,#6,#7 \rangle}
\newcommand{\csummary}[8]{\langle #1,#2,#3,#5,#6,#8 \rangle}
\newcommand{\dsumm}{a^d}
\newcommand{\unprotectedwrite}{\mathrm{UnprotectedW}}
\newcommand{\readwriterace}{\mathrm{RWRace}}
\newcommand{\uwrite}[1]{\unprotectedwrite(#1)}
\newcommand{\rwrace}[2]{\readwriterace(#1,#2)}
\newcommand{\bugsad}{\mathcal{B}} %bugs abtract domain
\newcommand{\bug}{b} % bug
\newcommand{\bugset}{B} % set of bugs
\newcommand{\patch}{p}
\newcommand{\act}{act}
\newcommand{\fpatch}{\widehat{\patch}}
\newcommand{\fact}{\widehat{\act}}
\newcommand{\patchset}{P}
\newcommand{\stmt}{s}
\newcommand{\snapshot}{a}
\newcommand{\algo}[1]{\textsc{#1}}
% Program keywords specific for concurrency
\newcommand{\sync}[1]{{\lstinline[basicstyle=\small\ttfamily]{synchronized(#1)} }}
\newcommand{\simil}{\simeq}
\newcommand{\rwbug}{Read/Write}
\newcommand{\uwbug}{Unprotected Write}
\newcommand{\acomment}[1]{{\color{gray}#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Colours and remarks
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\definecolor{pblue}{rgb}{0.13,0.13,1}
\definecolor{pgreen}{rgb}{0,0.5,0}
\definecolor{pred}{rgb}{0.9,0,0}
\definecolor{pgrey}{rgb}{0.46,0.45,0.48}

\definecolor{ckeyword}{HTML}{7F0055}
\definecolor{ccomment}{HTML}{3F7F5F}
\definecolor{cnumber}{HTML}{2A0099}
\definecolor{darkgreen}{HTML}{008000}


\newcommand{\todo}[1]{\mute{\textcolor{red}{(TODO: {#1})}}}
\newcommand{\ac}[1]{\mute{\textcolor{ACMPurple}{(Andreea: {#1})}}}
\newcommand{\is}[1]{\mute{\textcolor{ACMBlue}{(Ilya: {#1})}}}
\newcommand{\ar}[1]{\mute{\textcolor{ACMDarkBlue}{(Abhik: {#1})}}}
\newcommand{\at}[1]{\mute{\textcolor{darkgreen}{(Abhishek: {#1})}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Listings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Java listing

\lstdefinelanguage{Java}{
  keywords={new, return, public, this, if, else, try, then, private,
    push, pop, unlock, while, throw,
    synchronized, final, class, case, switch, new, for, protected, extends, implements, import,
    volatile, null, static},
  ndkeywords={bool, int, void, double, float},
  moredelim=[il][\textcolor{ACMOrange}]{$$},
  string=[b]",
  showspaces=false,
  showtabs=false,
  breaklines=true,
  showstringspaces=false,
  breakatwhitespace=true,
  lineskip=-0.0pt,
  morecomment=[l]{//}, % l is for line comment
  morecomment=[s]{/*}{*/}, % s is for start and end delimiter
  basewidth={0.54em, 0.4em},%
  basicstyle=\footnotesize\ttfamily,
  keywordstyle={\color{ACMPurple}\ttfamily\bfseries},
  ndkeywordstyle={\color{ACMDarkBlue}\ttfamily\bfseries},
  commentstyle={\color{ccomment}\itshape},
  stringstyle=\color{darkgreen},
  xleftmargin=1em,
  moredelim=[is][\textcolor{pgrey}]{\%\%}{\%\%}
}

\lstdefinestyle{numbering}{
  numbers=left,
  numberstyle={\scriptsize\color{cnumber}\sf},
  xleftmargin=2em
}

\newcommand{\jcode}[1]{\lstinline[language=Java,basicstyle=\small\ttfamily]{#1}}
\newcommand{\code}[1]{\jcode{#1}}

\lstset{
  language=Java,
 %  backgroundcolor=\color{backcolour},   
 % aboveskip=-1mm,
 % belowskip=-1mm,
  showstringspaces=false,
  columns=flexible,
  basicstyle={\footnotesize\ttfamily},
 % numbers=left,
  numberstyle=\tiny\color{black},
  numbersep=3pt,
  % keywordstyle=\color{blue},
  commentstyle=\color{gray},
  stringstyle=\color{mauve},
 breaklines=true,
  breakatwhitespace=true,
  tabsize=3,
  escapeinside={*}{*},
  morekeywords={String, Intent}
} 
\newcommand{\powerset}{\mathscr{P}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Concurrency-fix related 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\owned{\mathrm{Owned}}
\def\unowned{\mathrm{Unowned}}
\newcommand{\ownedif}[1]{\mathrm{OwnedIf}(#1)}
\newcommand{\modif}{\mathit{md}}
\newcommand{\mcode}[1]{\text{\lstinline[language=Java,basicstyle=\small\ttfamily]{#1}}}
\newcommand{\mmcode}[1]{\text{\lstinline[language=Java,basicstyle=\footnotesize\ttfamily]{#1}}}

\newcommand{\race}{\mathit{race}}
\newcommand{\wrace}{\mathit{unprotected\_write}}
\newcommand{\cls}{\it{cls}}
\newcommand{\acc}{\it{acc}}
\newcommand{\mthd}{\it{mthd}}
\newcommand{\idn}[1]{\mathit{#1}}
\newcommand{\dsl}{RFDSL\xspace}


==> tab-large.tex <==
\begin{table}[]

%\todo{Add numbers of concurrency-related commits in these projects.}
\begin{adjustbox}{width=\linewidth}
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{Project Name} & \textbf{\#Stars} & \textbf{\#Forks} & \textbf{\#Commits} & \textbf{\#matching Commits} \\ \hline
Apache Tomcat         & 4.7k             & 3.2k             & 22.36k   & 456            \\ \hline
Guava         & 38.3k             & 8.6k             & 5.3k    &  187         \\ \hline
%RxJava         & 43.2k             & 7.2k             & 5.7k   &  187         \\ \hline
%OkHttp         & 37.9k             & 8.1k             & 4.6k   &  0       \\ \hline
\end{tabular}
\end{adjustbox}
\caption{Large-Scale Projects}
\label{tab:realprojects}
\end{table} 


==> tab-racerd.tex <==
\begin{adjustbox}{width=\width}
\centering
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
{\color[HTML]{000000} \textbf{Id}} & {\color[HTML]{000000} \textbf{Program Name}} & {\color[HTML]{000000} \textbf{type}} & {\color[HTML]{000000} \textbf{RacerD Detection}}  \\ \hline
1                                  & account                                                                              & AV                  & Fail                                                                                                                           \\ \hline
2                                  & accountsubtype                                                                   & AV                  & Fail                                                                                                                           \\ \hline
3                                  & airline                                                                          & AV                  & Success                                                                                                                           \\ \hline
4                                  & alarmclock                                                                       & DR                    & Success                                                                                                                                  \\ \hline
5                                  & atmoerror                                                                         & DR                  & Success                                                                                                                          \\ \hline
6                                  & buggyprogram                                                                     & AV                  & Success                                                                                                                            \\ \hline
7                                  & checkfield                                                                        & AV                  & Success                                                                                                                           \\ \hline
8                                  & consisitency                                                                      & CB                  & Success                                                                                                                           \\ \hline
9                                  & critical                                                                         & AV                  & Success                                                                                                                          \\ \hline
10                                 & datarace                                                                          & DR                  & Success                                                                                                                          \\ \hline
11                                 & even                                                                              & AV                  & Success                                                                                                                           \\ \hline
12                                 & hashcodetest                                                                   & AV                  & Success                                                                                                                           \\ \hline
13                                 & linkedlist                                                                       & AV                  & Success                                                                                                                            \\ \hline
14                                 & mergesort                                                                        & AV                  & Success                                                                                                                               \\ \hline
15                                 & pingpong                                                                         & DR                  & Success                                                                                                                          \\ \hline
16                                 & ProducerComsumer                                                                 & AV                    & Success                                                                                                                              \\ \hline
17                                 & reorder2                                                                         & CB                  & Success                                                                                                                            \\ \hline
18                                 & store                                                                             & AV                  & Success                                                                                                                           \\ \hline
19                                 & stringbuffer                                                                    & AV                  & Fail                                                                                                                            \\ \hline
20                                 & wrongLock                                                                         & AV                  & Success                                                                                                                         \\ \hline
21                                 & wrongLock2                                                                       & DR                  & Success                                                                                                                           \\ \hline
\end{tabular}
\end{adjustbox}


==> tab-selection.tex <==
\begin{table}[]
\caption{Subject Apps. AV -- Atomicity Violation, CB -- Consistency bug, DR -- Data Race} 
\label{tab:rq1}
%\vspace{2mm}
\begin{adjustbox}{width=\width}
\centering
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
 {\color[HTML]{000000} \textbf{Program Name}} & {\color[HTML]{000000} \textbf{\#line}} & {\color[HTML]{000000} \textbf{type}} & {\color[HTML]{000000} \textbf{Benchmarks}}  \\ \hline
                                   account                                      & 102                                    & AV                  & PECAN, JaConTeBe, PFix                                                                                                                           \\ \hline
                                   accountsubtype                               & 138                                    & AV                  & PFix                                                                                                                           \\ \hline
                                   airline                                      & 51                                     & AV                  & JaConTeBe, PFix                                                                                                                           \\ \hline
                                   alarmclock                                   & 206                                    & DR                    & JaConTeBe, PFix                                                                                                                                  \\ \hline
                                   allocation vector                            & 114                                    & DR                    & JaConTeBe                                                                                                                                  \\ \hline
                                   atmoerror                                    & 48                                     & DR                  & PFix                                                                                                                          \\ \hline
                                   buggyprogram                                 & 258                                    & AV                  & PECAN, PFix                                                                                                                            \\ \hline
                                   checkfield                                   & 41                                     & AV                  & PFix                                                                                                                           \\ \hline
                                   consisitency                                 & 28                                     & CB                  & PFix                                                                                                                           \\ \hline
                                   critical                                     & 56                                     & AV                  & PECAN, JaConTeBe, PFix                                                                                                                          \\ \hline
                                  datarace                                     & 90                                     & DR                  & PFix                                                                                                                          \\ \hline
                                  even                                         & 49                                     & AV                  & PFix                                                                                                                           \\ \hline
                                  hashcodetest                                 & 1258                                   & AV                  & PFix                                                                                                                           \\ \hline
                                linkedlist                                   & 204                                    & AV                  & PECAN, JaConTeBe, PFix                                                                                                                            \\ \hline
                                  Manager                                      & 130                                    & AV                  & PECAN                                                                                                                            \\ \hline
                                  mergesort                                    & 270                                    & AV                  & PECAN, PFix                                                                                                                               \\ \hline
                                  pingpong                                     & 130                                    & DR                  & PFix                                                                                                                          \\ \hline
                                 ProducerComsumer                             & 144                                    & AV                    & PFix                                                                                                                              \\ \hline
                                  reorder2                                     & 135                                    & CB                  & JaConTeBe, PFix                                                                                                                            \\ \hline
                                  store                                        & 44                                     & AV                  & PFix                                                                                                                           \\ \hline
                                  stringbuffer                                 & 416                                    & AV                  & PECAN, PFix                                                                                                                             \\ \hline
                                  wrongLock                                    & 73                                     & AV                  & JaConTeBe, PFix                                                                                                                         \\ \hline
                                 wrongLock2                                   & 36                                     & DR                  & PFix                                                                                                                           \\ \hline
\end{tabular}
%\end{adjustbox}
\end{table}

